Latent Space Symmetry Discovery

Equivariant neural networks require explicit knowledge of the symmetry group. Automatic symmetry discovery methods aim to relax this constraint and learn invariance and equivariance from data. However, existing symmetry discovery methods are limited to simple linear symmetries and cannot handle the complexity of real-world data. We propose a novel generative model, Latent LieGAN (LaLiGAN), which can discover symmetries of nonlinear group actions. It learns a mapping from the data space to a latent space where the symmetries become linear and simultaneously discovers symmetries in the latent space. Theoretically, we show that our model can express nonlinear symmetries under some conditions about the group action. Experimentally, we demonstrate that our method can accurately discover the intrinsic symmetry in high-dimensional dynamical systems. LaLiGAN also results in a well-structured latent space that is useful for downstream tasks including equation discovery and long-term forecasting.

==> sec/exp2.tex <==
\subsection{Nonlinear Ordinary Differential Equations}


\ryu{re-group the experiments. first introduce different dynamical systems , then talk about equation discovery and long term forecasting. If we don't have space, move Figure 7 or 8 to appendix}

The  reaction-diffusion system is an example of low-dimensional latent symmetry in high-dimensional observations. In fact, the absence of linear symmetry is not exclusive in high-dimensional systems. Here we investigate two low-dimensional dynamics, where their nonlinear evolution prevents any kind of linear symmetry, but our method can still discover meaningful symmetries in the latent space.
\paragraph{Nonlinear pendulum.}
The movement of a simple pendulum can be described by $\dot q=p,\ \dot p=-\omega^2\sin(q)$, with $\omega$ being the natural frequency and $q$ and $p$ the angular displacement and angular momentum. In our experiment, we use $\omega=1$.

\paragraph{Lotka-Volterra System.}
The Lotka-Volterra equations are a pair of nonlinear ODEs that characterize the dynamics of predator-prey interaction. We consider the canonical form of the equations,
$
    \dot p = a - b e ^ q , \ 
    \dot q = c e ^ p - d
$,
where $p$ and $q$ are the logarithm population densities of prey and predator, and the parameters $a, b, c, d$ indicate the growth and death rate of the two populations.
In our experiment, we use $a=2/3, b=4/3, c=d=1$.

Figure \ref{fig:ode-original} shows the trajectories of $(p,q)\in\mathbb R^2$ generated from different initial conditions in these two systems. These nonlinear dynamics do not possess any global linear symmetry in the original observation space. We apply \ours{} on each system to identify a coordinate transformation that takes the original coordinates to a symmetric embedding space.

\begin{figure}[ht]
    \centering
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/pendulum/original.png}
    %     \caption{}
    %     \label{fig:pd-original}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/pendulum/latent.png}
    %     \caption{}
    %     \label{fig:pd-latent}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/pendulum/original-transformed.png}
    %     \caption{}
    %     \label{fig:pd-transformed}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/pendulum/original-transformed-linear.png}
    %     \caption{}
    %     \label{fig:pd-transformed-lin}
    % \end{subfigure}

    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/lv/original.png}
    %     \caption{}
    %     \label{fig:lv-original}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/lv/latent.png}
    %     \caption{}
    %     \label{fig:lv-latent}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/lv/original-transformed.png}
    %     \caption{}
    %     \label{fig:lv-transformed}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.2\textwidth}
    %     \includegraphics[width=\textwidth]{figs/lv/original-transformed-linear.png}
    %     \caption{}
    %     \label{fig:lv-transformed-lin}
    % \end{subfigure}

    % \begin{minipage}{0.3\textwidth}
    %     \subcaption*{Pendulum}
    %     \subcaption*{L-V}
    % \end{minipage}

    \begin{subfigure}{.195\textwidth}
        \includegraphics[width=\textwidth]{figs/ode/ode-original.png}
        \caption{}
        \label{fig:ode-original}
    \end{subfigure}
    \begin{subfigure}{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/ode/ode-latent.png}
        \caption{}
        \label{fig:ode-latent}
    \end{subfigure}
    \begin{subfigure}{.2\textwidth}
        \includegraphics[width=\textwidth]{figs/ode/ode-original-transformed.png}
        \caption{}
        \label{fig:ode-transformed}
    \end{subfigure}
    \begin{subfigure}{.195\textwidth}
        \includegraphics[width=\textwidth]{figs/ode/ode-original-transformed-linear.png}
        \caption{}
        \label{fig:ode-transformed-lin}
    \end{subfigure}
    
    \caption{Latent symmetry discovery in nonlinear pendulum (upper) and Lotka-Volterra equations (lower). (a) Original trajectories of the systems. The color of each trajectory corresponds to its Hamiltonian. (b) The trajectories are mapped to a symmetric latent space. (c) Original trajectories transformed by \ours{}. (d) Original trajectories transformed by linear LieGAN.}
    \label{fig:sym-dis-nd}
\end{figure}

Figure \ref{fig:ode-latent} shows the trajectories of these two systems in the latent space, with the discovered symmetries
$L_{\text{pendulum}}=\begin{bmatrix}
    0 & -5.24 \\
    2.16 & 0
\end{bmatrix}$ and $L_{\text{LV}}=\begin{bmatrix}
    0 & 2.43 \\
    -2.74 & 0
\end{bmatrix}$. These correspond to rotation symmetries up to certain scaling in the two latent dimensions. To verify their validity, we use the learned symmetries to transform all data points within each original trajectory simultaneously, as is shown in figure \ref{fig:ode-transformed}. Each trajectory is transformed from the original trajectory of the same color in figure \ref{fig:ode-original}. While each individual data point is taken into a new position, the overall trajectories remain similar before and after transformation, suggesting that the discovered transformations are indeed the symmetries of these systems. In contrast, the linear symmetries learned by LieGAN do not preserve valid trajectories in the observation space, as shown in figure \ref{fig:ode-transformed-lin}.

We also conduct the same experiments of equation discovery and long-term forecasting as for the reaction-diffusion system. While these systems have simple closed-form governing equations in the observation space, we find that discovering a latent space with learnable symmetry can still be beneficial. The symmetry enforces linear governing equations and leads to reduced error accumulation in long-term forecasting. The detailed results are available in Appendix \ref{sec:supp-ode}.


==> sec/notes-eed.tex <==
\newpage
\section{Equivariant equation discovery}
Say we want to discover the governing equation from a dynamical system:
\begin{equation}
    \dot{\mathbf z}= \mathbf h(\mathbf z),\ \mathbf z\in\mathbb R^m
\end{equation}
If the prediction function $\mathbf z_{t+1}=\mathbf f(\mathbf z_t)$ is equivariant to a group $G$ through its linear representation $\pi:G\rightarrow \mathrm{GL}(m)$, i.e.
\begin{align}
    \pi(g)\mathbf z_{t+1}=\mathbf f(\pi(g)\mathbf z_t)
\end{align}
\nd{In general it could be $\pi_1(g)z_{t+1}= f(\pi_2(g)z_t)$ or even $\rho(g,z_t)z_{t+1}=f(\pi(g)z_t)$. 
Also, no need to switch from $\dot{z}$ to $z_{t+1}$. 
We can have $\pi_1(g)\dot{z}= h(\pi_2(g)z)$.
}
what can we say about the operator $\mathbf h$ in the governing equation?

First we need to establish the connection between $\mathbf f$ and $\mathbf h$. Consider the most simple case where the time-discretized data is generated by the forward Euler method. We have
\begin{align}
    &\mathbf z_{t+1}=\mathbf f(\mathbf z_t)=\mathbf z_t+\mathbf h(\mathbf z_t)\Delta t\\
    \Rightarrow&\pi(g)\mathbf z_{t+1}=\pi(g)\mathbf z_t+\mathbf h(\pi(g)\mathbf z_t))\Delta t\\
    \Rightarrow&(\pi(g)-I)\mathbf z_{t+1}=(\pi(g)-I)\mathbf z_t+[\mathbf h(\pi(g)\mathbf z_t)-\mathbf h(\mathbf z_t)]\Delta t\\
    \Rightarrow&(\pi(g)-I)\mathbf h(\mathbf z_t)=\mathbf h(\pi(g)\mathbf z_t)-\mathbf h(\mathbf z_t),\ \forall g\in G,\ \mathbf z_t\in\mathcal Z\label{eq:eed-1}
\end{align}
\yjk{Actually if we assume equivariance of $\mathbf h$ instead of $\mathbf f$, we will have exactly the same result.}

For a connected matrix Lie group, we may write $\pi(g)=\exp(w^iL_i)$. By Taylor expansion we have $\pi(g)\approx I+\epsilon^iL_i$ when $\epsilon\in\delta_0$. Then, $\mathbf h(\pi(g)\mathbf z_t)-\mathbf h(\mathbf z_t)=\mathbf J_\mathbf h(\mathbf z_t)\epsilon^iL_i\mathbf z_t+O(\epsilon^2)$. With these first order approximations eq. \eqref{eq:eed-1} becomes
\begin{equation}
    (L\circ \mathbf h)(\mathbf z)=\mathbf J_\mathbf h(\mathbf z)\cdot L\mathbf z
\end{equation}
\nd{Alternative derivation:
Suppose we are looking for equivariances of the form 
\[ \pi(g)\dot{z} = h(\pi(g) z)\]
consider infinitesimal $\pi(g) = I+\epsilon^i L_i$. 
We get your equation 
\[h(\pi(g)z) =h(z) +\epsilon^i J_h(z) \cdot L_i z \]
Similarly, $\pi(g)\dot{z} = \dot{z}+ \epsilon L 
 \dot{z}$. 
Setting the two side equal we have 
\[L\dot{z} = J_h(z) \cdot L z\]
When $h(z) = Kz$, we get $L\dot{z} = LKz = KLz$. 
Now, note that if we had $\pi_2(g)\dot{z} = h(\pi_1(g) z)$, $K$ needs to be an intertwiner because from $\pi_2(g) = I+\epsilon d\pi_2(L)$ we get 
\begin{align}
    d\pi_2(L)\dot{z} &= J_h(z) \cdot d\pi_1(L) z\cr 
    h(z) = Kz, \quad &\Rightarrow  d\pi_2(L)K= K d\pi_1(L)
\end{align}
}
for any Lie algebra element $L\in\mathfrak g$. Specifically, this holds for the discovered Lie algebra basis $L_i$.

If $\mathbf h$ is a linear operator, i.e. $\mathbf h(\mathbf z)=K\mathbf z,\ K\in\mathbb R^{m\times m}$, then $K$ must commute with $L$, i.e. $KL=LK$. Such constraint can potentially be incorporated into equation discovery algorithms such as SINDy. \yjk{Maybe we can solve the constraints like \citet{emlp} did in Equivariant MLP.}

For example, let $L=\begin{bmatrix}
    0 & -1 \\ 1 & 0
\end{bmatrix}$. $KL=LK$ implies $K\in\Big\{\begin{bmatrix}
    a & b \\ -b & a
\end{bmatrix}\Big |\ a,b\in\mathbb R\Big\}$.

In our previous example of 3D latent space for RD system, the result does not strictly satisfy the commutative property:
\begin{equation}
    L=\begin{bmatrix}
        -0.03 & 2.00 & -1.97 \\ -2.09 & -0.02 & 2.37 \\ 2.02 & -2.33 & 0.03
    \end{bmatrix},\ K=\begin{bmatrix}
        0 & 0.43 & -0.53 \\ -0.51 & 0 & 0.66 \\ 0.47 & -0.52 & 0
    \end{bmatrix},\ 
    [K,L]=\begin{bmatrix}
        -0.02 & 0.21 & -0.33 \\ 0.22 & -0.43 & -0.07 \\ -0.13 & 0.10 & 0.45
    \end{bmatrix}
\end{equation}

\nd{I think they actually do commute. It looks like approximately 
\begin{align}
    L = 2 \begin{bmatrix}
        0 & 1&-1\\
        -1&0&1\\
        1&-1&0
    \end{bmatrix} = 4K, \quad [K,L]=0
\end{align}
Also, $L$ is the Lie algebra of $SO(2)$ in a tilted plane in 3D (since it's antisymmetric), and those rotations really represent the time translations, so we must have $L\propto K$. 
}

More generally, $\mathbf h$ is constructed from a library of measurement functions, i.e. $\mathbf h(\mathbf z)=\mathbf \Xi\mathbf \Theta(\mathbf z),\ \mathbf \Xi\in\mathbb R^{m\times p},\ \mathbf{\Theta(z)}\in\mathbb R^p$. We ensure that the linear terms are included in $\mathbf \Theta$. The learnable parameters are $\mathbf \Xi$. We have
\begin{equation}
    L\mathbf{\Xi\Theta(z)}=\mathbf{\Xi J_\Theta(z)}\cdot L\mathbf z
    \label{eq:eed-2}
\end{equation}
% \yjk{This should hold true for all possible $\mathbf z$'s. The linear case is simple because the Jacobian is constant. How do we deal with a varying Jacobian? I doubt whether there exist higher-order polynomials (or other functions) that satisfy this constraint. See the following proof.}

% For example, let $L=\begin{bmatrix}
%     0 & -1 \\ 1 & 0
% \end{bmatrix}$, $m=2$ and  $\mathbf{\Theta(z)}=[1, z_1, z_2, z_1^2, z_1z_2, z_2^2]^T$. We have
% \begin{equation}
%     L\mathbf\Xi\begin{bmatrix}
%         1 \\ z_1 \\ z_2 \\ z_1^2 \\ z_1z_2 \\ z_2^2
%     \end{bmatrix}=\mathbf\Xi \begin{bmatrix}
%         0 & 0 \\ 1 & 0 \\ 0 & 1 \\ 2z_1 & 0 \\ z_2 & z_1 \\ 0 & 2z_2
%     \end{bmatrix}L\mathbf z=\mathbf\Xi\begin{bmatrix}
%         0 \\ -z_2 \\ z_1 \\ -2z_1z_2 \\ z_1^2-z_2^2 \\ 2z_1z_2
%     \end{bmatrix}
% \end{equation}
% \nd{I think this is because of your choice of basis functions $\Theta(z)$. 
% Note that your equation is really 
% \begin{align}
%     L\dot{z} = Lz \cdot \nabla h(z)
% \end{align}
% The linear operator $\hat{L} = Lz\cdot \nabla$ has its own eigenbasis, which are a set of functions satisfying $\hat{L}(z) F(z) = \lambda F(z)$. 
% For example, spehrical harmonics are the eigenfunctions of the operator $\hat{L}^2 $ and $\hat{L}_z$ for basis $L_i \in so(3)$. 
% So, I think if you had chosen the right basis for $\Theta(z)$ (which I think are the Legendre polynomials) you would not reach this conclusion.
% }
% After some calculations we can conclude that the coefficients for quadratic terms have to be zero.

% To prove that $\mathbf h$ is linear, we can substitute $L\mathbf z=L'\mathbf{\Theta(z)}$ into \eqref{eq:eed-2} (if $\mathbf \Theta(\mathbf z)$ contains linear terms), where $L'\in\mathbb R^{m\times p}$ is just an extension of $L$ with zero columns, so that
% \begin{equation}
%     L\mathbf\Xi=\mathbf{\Xi J_\Theta(z)}L'
% \end{equation}
% which means $\mathbf{\Xi J_\Theta(z)}L'$ does not depend on $\mathbf z$. If $\mathbf{\Theta}_i$ is not linear with regard to $z_j$, then $\mathbf{(J_\Theta)}_{ij}$ depends on $z_{j}$. Then there are two possibilities: (i) $L'_{j\cdot}=\mathbf 0$, and thus $L_{j\cdot}=\mathbf 0$; (ii) $\mathbf\Xi_{\cdot i}=\mathbf 0$. In other words, either there is no symmetry at all concerning this dimension, or this dimension is totally irrelevant to the governing equation of the dynamics.

% \yjk{Actually it is wrong to conclude that $\mathbf{\Xi J_\Theta(z)}L'$ does not depend on $\mathbf z$. Consider the following example.}

For example, let $L=\begin{bmatrix}
    2 & 0 \\ 0 & 1
\end{bmatrix}$, $m=2$, $\mathbf\Xi=\begin{bmatrix}
    0 & 0 & 1 \\ 0 & k & 0
\end{bmatrix}$ and $\mathbf{\Theta(z)}=[z_1, z_2, z_2^2]^T$. Equivalently,
\begin{equation}
    \begin{cases}
        \dot z_1=z_2^2 \\
        \dot z_2=kz_2
    \end{cases}
\end{equation}

Equation \eqref{eq:eed-2} translates to 
\begin{equation}
    \begin{bmatrix}
        0 & 0 & 2 \\ 0 & k & 0
    \end{bmatrix}\begin{bmatrix}
        z_1 \\ z_2 \\ z_2^2
    \end{bmatrix}=\begin{bmatrix}
        0 & 0 & 1 \\ 0 & k & 0
    \end{bmatrix}\begin{bmatrix}
        1 & 0 \\ 0 & 1 \\ 0 & 2z_2
    \end{bmatrix}\begin{bmatrix}
        2 & 0 & 0 \\ 0 & 1 & 0
    \end{bmatrix}\begin{bmatrix}
        z_1 \\ z_2 \\ z_2^2
    \end{bmatrix}
\end{equation}
which actually holds, where we cannot simply eliminate the $\mathbf{\Theta(z)}$ at the end because $\mathbf{J_\Theta(z)}$ interacts with it.

One can easily verify that $L$ represents a scaling symmetry, $z_1\rightarrow a^2z_1,\ z_2\rightarrow az_2$, which is indeed the symmetry of this system.

In order to solve the symmetry constraint for a nonlinear system, we need to eliminate any $\mathbf z$ in the formula. Let's define a symbolic map $\mathcal M_{\mathbf \Theta}:(\mathbb R^m\rightarrow \mathbb R^p)\rightarrow \mathbb R^{p\times p}$, which basically maps a function to its coordinate in the function space spanned by $\mathbf\Theta$. Of course $\mathcal M_{\mathbf \Theta}(\mathbf\Theta)=I_p$. Thus we have the constraint
\begin{equation}
    L\mathbf\Xi=\mathbf\Xi\mathcal M_{\mathbf\Theta}(\mathbf{J_\Theta(z)}\cdot L\mathbf z)
\end{equation}

In the previous example, this translates to
\begin{equation}
    \begin{bmatrix}
        2 &  \\  & 1
    \end{bmatrix}\mathbf\Xi=\mathbf\Xi\begin{bmatrix}
        2 & & \\ & 1 & \\ & & 2
    \end{bmatrix}
\end{equation}
which implies $\mathbf{\Xi}\in \Big\{\begin{bmatrix}
    a & 0 & b \\ 0 & c & 0
\end{bmatrix}\Big|a,b,c\in\mathbb R\Big\}$.


\newpage
\subsection{Implicit Formulation}
Assume that the governing equation is written in an implicit form \citep{sindy-pi}:
\begin{equation}
    \mathbf{ f(z,\dot z) = 0}, \mathbf z \in \mathbb R^m, \mathbf f: \mathbb R^m \rightarrow \mathbb R^m
\end{equation}

The form of the governing equation, whether explicit or implicit, does not affect our symmetry discovery algorithm. The discovered equivariance, if any, can be similarly formulated as
\begin{equation}
    \mathbf{ f(z }_t, \mathbf{ \dot z}_t) = \mathbf 0 \Rightarrow \mathbf f ( g \mathbf z_t , g \mathbf{ \dot z }_t ) = \mathbf 0
\end{equation}

We may write $g = \exp (w^iL_i)$ for a connected matrix Lie group and also $g \approx I + \epsilon^i L_i$ when $\epsilon \in \delta_0$. Then, the equivariance constraint becomes
\begin{align}
    \frac{\partial \mathbf f ( g \mathbf z , g \mathbf{ \dot z } )}{\partial \epsilon_i}
    = &
    \frac{\partial \mathbf f ( g \mathbf z , g \mathbf{ \dot z } )}{\partial (g \mathbf z)} \frac{\partial (g \mathbf z)}{\partial \epsilon_i}
    +
    \frac{\partial \mathbf f ( g \mathbf z , g \mathbf{ \dot z } )}{\partial (g \mathbf{\dot z})} \frac{\partial (g \mathbf{\dot z}))}{\partial \epsilon_i} \\
    = &
    \frac{\partial \mathbf f}{\partial \mathbf z}L_i \mathbf z + \frac{\partial \mathbf f}{\partial \mathbf{\dot z} }L_i \mathbf{ \dot z }
\end{align}

If $\mathbf f$ is expressed in terms of the function space basis as $\mathbf {f(z, \dot z)} = \mathbf \Xi \mathbf {\Theta (z, \dot z)}$, we have

\begin{equation}
    \mathbf \Xi (\mathbf{ J_\Theta (z)} L_i \mathbf z + \mathbf{ J_\Theta (\dot z)} L_i \mathbf { \dot z } ) = \mathbf 0
\end{equation}

Is there a proper function space that is closed under the symmetry operator (similar to the polynomial space in the explicit formulation)? Are there any interesting examples with nontrivial symmetries?

==> sec/notes.tex <==
\section{Representation vs nonlinear group action}\label{sec:nonlinear-group-action}

Given an abstract group $G$, a representation $\pi:G\to \GL(n,F)$ maps the group product $\cdot $ to the matrix product, such that for $g_1,g_2 \in G$, $g_1\cdot g_2 = \pi(g_1)\pi(g_2)$. 
The representation $\pi$ gives a natural linear action on the vector space $\mathcal{V}=F^n$ via the linear matrix multiplication on column vectors from the left, meaning for $x\in \mathcal{V}$, we can define $g\cdot x = \pi(g)x$. 

Now assume we want a group to act nonlinearly on the vector space $\mathcal{V}$. 
%A representation defines a linear action, but we can generalize it to functions with a nonlinear actions. %, called an \textit{equivariance}. 
A general nonlinear action is defined by $\pi': G\times \mathcal{V}\to \mathcal{V}$ %is called an equivariance if it 
satisfying 
\begin{align}
    %g \cdot x &= \pi'(g, x)\\
    %g_2 \cdot(g_1 \cdot x)& =
    \pi'(g_2, \pi'(g_1,x))= \pi'(g_2\cdot g_1, x) 
    \label{eq:G-act-nonlin}
\end{align}
We often denote $g \cdot x = \pi'(g, x)$.

We want to learn nonlinear group actions.
Our proposal is to encode the nonlinear function $\pi'$ in a specific way using an autoencoder. 
We are not claiming that our proposal is the most general form of nonlinear action. 
We propose to encode $\pi'$ using a representation $\pi:G \to \GL(m)$ and an encoder $\phi: \R^n \to \R^m$ and decoder function $\psi: \R^m \to \R^n$. 
Assume that we have a dataset $\mathcal{X}\subset \mathcal{V} $  whose true dimensionality $m$ is lower than the dimensionality $n$ of $\mathcal{V}$. 
Assume that the encoder/decoder function are such that for all $x\in \mathcal{X}$ 
\begin{align}
    (\psi\circ\phi)(x) &= x + \delta x 
    \label{eq:AE-delta}
\end{align}
\nd{$\psi$ and $\phi$ are a bit difficult to distinguish and remember their roles. $E$ and $D$ would be easier to follow.}
where $\|\delta x\| < \eta $ is a  small bounded error. 
First, assume $\eta=0$, meaning autoencoder is perfect, that is, has no error. Then the decoder is an exact left inverse to the encoder. 
Define the set of latent embeddings as $\mathcal{Z} = \{z=\phi(x): x \in \mathcal{X} \}$. 
For a perfect autoencoder (AE) and $z=\phi(x)\in \mathcal{Z}$ we have 
\begin{align}
    (\psi\circ\phi)(x) &= x \cr 
   (\phi\circ\psi)(z) &= (\phi\circ\psi\circ\phi)(x) = z   
\end{align}
meaning, on the subspaces $\mathcal{X}\subset F^n$ and $\mathcal{Z}\subset F^m$, the functions $\phi$ and $\psi$ are inverse of each other.

Now we propose to define a nonlinear action of $G $ on $\mathcal{X}$ as $\pi': G\times \mathcal{X} \to \mathcal{X}$ in the following form. 
The existence of this action requires that $\mathcal{Z}$ is invariant (symmetric) under the linear action of $G$ using a representation $\pi: G \to F^n$, meaning
\begin{align}
    \forall z \in \mathcal{Z}, g\in G: \  \pi(g)z \in \mathcal{Z} 
\end{align}
When this symmetry on $\mathcal{Z}$ and a perfect AE for $\mathcal{X} \to \mathcal{Z}\to \mathcal{X}$ exist, we can define a nonlinear action of $G$ on $\mathcal{X}$ as follows. 
For $g\in G$ and $x\in \mathcal{X}$
%
\begin{align}
    \pi'(g, x) &\equiv \psi(\pi(g) \phi(x)).  
\end{align}
We can check that this satisfies the group action properties \eqref{eq:G-act-nonlin}
\begin{align}
    \pi'(g_2, \pi'(g_1, x))&= \psi(\pi(g_2) \phi(g_1\cdot x))\cr 
    &=\psi(\pi(g_2) \phi(\psi(\pi(g_1) \phi(x)))) \cr 
    &=\psi(\pi(g_2) \pi(g_1) \phi(x)) \cr 
    &=\psi(\pi(g_2 g_1) \phi(x)) \cr 
    &=\pi'(g_2 g_1, x)
\end{align}

Where we used the assumption that $\mathcal{Z}$ is symmetric under $G$ to get $z_1 = \pi(g_1) \phi(x) \in \mathcal{Z}$ and $\phi(\psi(z_1)) = z_1$. 

Thus, our procedure can be used to define nonlinear group actions on a subset of a vector space. 

\nd{
Now we want to quantify the error in dynamics prediction with and without such symmetry prediction. 
For that we need to narrow down the problem and relation of symmetry to dynamics. 
The simplest case would be when the symmetry is the time translation (dynamics) itself. 
Also, the dynamics needs to be nonlinear in the original coordinates. 
But before worrying about the dynamics in the original space, what can we say when we have an imperfect, but good AE (i.e. small $1\gg \eta>0$, in an appropriate scale)?
So what we care about is how the error grows as we extrapolate farther in the future. 
First we need to see how the group action is affectedx by having imperfect AE, meaning when $\delta x\ne 0 $ in \eqref{eq:AE-delta}. 

}

\subsection{Universal Approximation of Nonlinear Group Action}\label{sec:uanga}
\begin{theorem}[Universal Approximation of Nonlinear Group Action]
    % For a general linear subgroup $G\leq\mathrm{GL}(k; \mathbb R)$, any nonlinear group action $\pi': G\rightarrow \mathcal C(\mathbb R^n, \mathbb R^n)$ can be approximated by the decomposition $\pi'(g)\approx\psi\circ\pi(g)\circ\phi$, where $\psi$ and $\phi$ are fixed neural networks and $\pi$ is a linear group representation.
    Let $G\leq\mathrm{GL}(k; \mathbb R)$ be a compact Lie group that acts smoothly, freely and properly on $X=\mathbb R^n$ via a continuous group action $\pi':G\times X\rightarrow X$. The group action can be approximated by the decomposition $\pi'(g,\cdot)\approx\psi\circ\pi(g)\circ\phi$, where $\psi$ and $\phi$ are fixed arbitrary-width neural networks with one hidden layer, and $\pi$ is a linear group representation, if it admits a simply connected orbit space $X/G$.
\end{theorem}

\begin{proof}
    We establish our theorem as a corollary of the Universal Approximation Theorem \citep{uat}, which states that any continuous function $f\in \mathcal C (\mathbb R^n, \mathbb R^m)$ can be approximated by a one-hidden-layer arbitrary-width neural network. We decompose the group action into explicitly defined continuous mappings between the input space and a latent space.

    The Quotient Manifold Theorem states that smooth, free, and proper group actions yield smooth manifolds as orbit spaces (\cite{lee2012smooth}, Theorem 21.10). More precisely, the orbit space $X/G$ has a unique smooth structure with a smooth submersion quotient map $s: X \rightarrow X/G$. Also, given that $X/G$ is simply connected, we can find a global continuous section $s': X/G \rightarrow X$ s.t. $s' \circ s$ is identity restricted on $S = \mathrm{img}_{s'} (X/G)$. The global section can be constructed by:
    \begin{enumerate}
        \item Fix a base point $p \in X/G$ and choose a point $\tilde p$ in the pre-image of $p$ under $s$, i.e. $s(\tilde p) = p$.
        \item For any other point $q \in X/G$, choose a path $\gamma$ in $X/G$ from $p$ to $q$.
        \item As $X/G$ is simply connected, $X$ is a universal cover of $X/G$, so that any path $\gamma$ in $X/G$ can be uniquely lifted to a path $\tilde\gamma$ in $X$ which starts at $\tilde p$ and ends at $\tilde q$.
        \item Define the section as $s': X/G \rightarrow X, q \mapsto \tilde q$.
    \end{enumerate}

    In addition, according to Whitney Embedding Theorem, the smooth manifold $X/G$ can be smoothly embedded in a higher-dimensional Euclidean space. Denote $t: X/G \rightarrow \mathbb R^p$ as one of the possible embeddings. We do not restrict the exact dimensionality of such an Euclidean space, as long as it enables us to represent any orbit with part of the latent space $\mathbb R^m$.
    
    % Let $\{[x_i]\}$ denote all the $\pi'(G)$-orbits in $X\subseteq\mathbb R^n$, and $\bar X=\{x_i\}$ are the representative elements. For each $x_i\in\bar X$, denote its $\pi'(G)$-stabilizer as $H_i=\mathrm{Stab}_{\pi'(G)}(x_i)$. We can choose a representative group element within each coset $[gH_i]\in G/H_i$. Denote $G_i$ as the set of all such representative elements. \yjk{Ideally $\bar X$ and any $G_i$ should be continuous.}

    Before defining the mapping from input to latent, we finally note that
    as $G\leq\mathrm{GL}(k; \mathbb R)$, we have a standard representation $\rho: G\rightarrow\mathbb R^{k\times k}$. Choose a $z_0\in\mathbb R^k$ s.t. $\mathrm{Stab}_{\rho(G)}(z_0)=\{\mathrm{id}\}$.
    % \yjk{Does such $z_0$ always exist?}

    Now we define $\pi_0:X \rightarrow \mathbb R^{k+p}, \pi'(g, s'(\tilde x)) \mapsto \text{concat} (\rho(g) z_0, t(\tilde x)), \forall \tilde x \in X/G, g\in G$, and we verify that this function is well defined.
    
    First, $X=\{\pi'(g, s'(\tilde x)) | \tilde x \in X/G, g \in G\}$, so that $\pi_0(x)$ is defined for any $x\in X$.
    
    Then, we need to make sure any $x\in X$ is written uniquely in the form of $x=\pi'(g) \tilde x$. $\forall \tilde {x_i}\not= \tilde{x_j}, g_i, g_j \in G, \pi'(g_i) \tilde {x_i} \not= \pi'(g_j) \tilde {x_j}$, because any two orbits never overlap in $X$.
    
    Also, $\forall g_1,g_2\in G, g_1\not= g_2$, as $\pi'$ acts freely, we have $\pi'(g_1) \tilde x\not=\pi'(g_2) \tilde x$.

    Next, we prove that $\pi_0$ defined this way is also continuous. As the value of $\pi_0$ is concatenated from two parts, it suffices to check the continuity for each component, i.e. $\pi_{01}(\pi'(g, s'(\tilde x))) = \rho(g) z_0$ and $\pi_{02}(\pi'(g, s'(\tilde x))) = t(\tilde x)$.

    For any open set $t(\tilde X) \subset \mathbb R^p$, the continuity of $t$ and $s$ guarantees that the inverse image, $(t \circ s)^{-1} t(\tilde X) = s^{-1} (\tilde X)$, is an open set. As $(s|_S)^{-1}=s'$, $s'(\tilde X)$ is an open set. The $\pi_{02}$ inverse image of $t(\tilde X)$ is $\bigcup_{g \in G}\pi'(g, s'(\tilde X))$. Note that $\forall g \in G, \pi'(g^{-1}, \cdot): X \rightarrow X$ is continuous, so that $\pi'(g, s'(\tilde X))$ is open. Therefore, the $\pi_{02}$ inverse image of any open set $t(\tilde X)$ is a union of open sets, which is also open, so that $\pi_{02}$ is continuous.

    Similarly, for any open set $\rho(U)z_0 \in \mathbb R^k$, $U$ is an open set because $\rho$ is simply the standard representation. The $\pi_{01}$ inverse image of $\rho(U)z_0$ is $\bigcup_{s'(\tilde x)} \pi'(U, s'(\tilde x))$. As the action of $G$ on $X$ is free, i.e. the stabilizer subgroup is trivial for all $x \in X$, we have $\pi'(\cdot, x): G \rightarrow X$ is an injective continuous map, so that its image of an open set is still open. Thus, we conclude that $\pi_{01}$ is also continuous.
    
    According to the Universal Approximation Theorem, there exists a one-hidden-layer arbitrary-width neural network $\phi$ that approximates the continuous $\pi_0$.

    Similarly, we define the inverse mapping $\pi_1: (\rho(g)z_0, t(\tilde x)) \mapsto \pi'(g, s'(\tilde x)), \forall \tilde x \in X/G, g\in G$. It is well-defined because the stabilizer of $z_0$ contains only identity, and also continuous because it is the inverse of $\pi_0$. According to the Universal Approximation Theorem, there exists another neural network $\psi$ that approximates $\pi_1$.

    Finally, defining $\pi(g)=\rho(g)$, we have
    \begin{align*}
        \pi'(g,x)=&\pi'(g, \pi'(g', s'(\tilde x)))\\
                  =&\pi'(gg', s'(\tilde x))\\
                  =&\pi_1(\rho(gg')z_0, t(\tilde x))\\
                  =&(\pi_1\circ\pi(g))(\rho(g')z_0, \tilde x)\\
                  =&(\pi_1\circ\pi(g)\circ\pi_0)(\pi'(g', s'(\tilde x))\\
                  \approx&(\psi\circ\pi(g)\circ\phi)(x),
                  \forall x\in X, g\in G
    \end{align*}
    \yjk{The intuition is to explicitly construct the mappings between input and latent space and use UAT to approximate them. The latent representation here is constructed as the concatenation of $\rho(g)z_0$ and $x_i$, which encodes transformation-relevant information (e.g. orientation of an image) and transformation-irrelevant information (e.g. whether it is a cat or a dog on the image). In practice, $x_i$ in the latent space can be replaced by another representation $\tilde x_i$, or simply $i$. This could be also none at all if all the variances in the dataset are described by the symmetry transformations alone, e.g. the rotating chair dataset with different orientations of only one object.
    
    The final step of the proof requires more explanation, since the approximation accuracy of the composition of functions is not guaranteed in the original UAT. We need to ensure that the neural network approximator is Lipschitz continuous, which is true if we use one layer NN with proper activation.}
\end{proof}

\nd{I think I have problem with whether $\pi$ always exists and whether it is ``invertible'' in the sense that $\pi_1\sim \pi_0^{-1}$. 
Maybe your assumptions about $x_i$ and its effect on $\pi'$ fixes that. 
But I think it should be: given $\pi'$ and $X$, it is always possible to construct such $\pi_0$.

Simple example where $\pi_0$ doesn't exist (I think): 
Let $G=\mathbb{Z}_2 = \{+1,-1\}$ under multiplication acting on $\mathbb{Z}_2$ itself.
Pick $x_i=1$. 
Let $\rho(g) = g \in \{\pm 1\}$, and $\pi'(g)(x)= g^2x$. 
Then, $\pi'(g)(x) = x$ because $g^2=1$ always. 
Hence, we cannot find any $\pi_0$ because $\pi_0(\pi'(+1)x) = +x$ and $\pi_0(\pi'(-1)x) = -x$, but because $\pi'(g)=1$ this is impossible (requires $+x=-x$ or $+1=-1$).  
Of course, this has issues with the stabilizers, but that's exactly my point. 
Your definition looks like for a general function $\pi'$ and arbitrary rep $\rho$, you assume there always exists a map $\pi_0$. 
I think we need to prove that for $\pi'$ satisfying the group action and $x_i$ defined above, we can always find a $\pi_0$.
}
\yjk{I think we need to define $\pi_0$ by enumerating over $X$, and then finding a unique decomposition $x=\pi'(g)x_i$ for each $x$, instead of enumerating over $g$ and $x_i$, which may cause problem. In your example, $x_1=+1$ and $x_2=-1$ are two different orbits, both with $G$ itself as stabilizer. So we choose the representative group elements as $G_1=G_2=\{+1\}$. Then we have unique decomposition for $x_1=+1$ and $x_2=-1$, and we define $\pi_0(+1)=\pi_0(\pi'(+1)\cdot +1)=\rho(+1)z_0$ and $\pi_0(-1)=\pi_0(\pi'(+1)\cdot -1)=\rho(+1)z_0$.}
\nd{But I think that wouldn't answer the main question of your theorem: Can \textit{any} group action be decomposed into the AE form?
So, even for group action like above you should be able to do it, with all its redundancy. 
I think you assumption is too general. 
I think there needs to be a relationship between $\pi'$ and $\rho$ for $\pi_0$ to exist. 
It may be a nonlinear generalization of Shur's lemma. 
Shur's lemma states that any rep can be block-diagonalized to have only irreps on the diagonal. 
This means for any rep $\pi'$ (linear action), $\pi'(g) = S^{-1} \rho(g) S$, where $\rho(g)$ is block diagonal and contains only irreps.
Shur's lemma also says that no $S$ exists that maps two different irreps (that's the definition of irreps, basically.
I think maybe a nonlinear version of Shur's lemma exists, meaning for any nonlienar action $\pi'(g, x) = \phi^{-1}(\rho(g)\phi(x)) $. 
And maybe such a nonlinear Shur's lemma would mean each $\pi'(g)$ can only be mapped to certain irreps (block of $\rho(g)$). 
My guess is it is no possible to map any $\pi'$ can be mapped to any arbitrary $\rho$. 
}

\subsection{Error growth}
\nd{Working on this still. We need to make the question clearer. What are we comparing against? What can we say about the case where we don't use symmetry discovery or have a nonlinear equation for a dynamics. 
I will use $E$ for encoder and $D$ for decoder, for ease of remembering. We can decide later to merge with previous section. }
We have the autoencoder 
\begin{align}
    (D\circ E)(x) = x+ \delta x, \qquad \|\delta x\| < \eta
\end{align}
and the group action 
\begin{align}
    g\cdot x = \rho(g,x) = D(\pi(g) E(x)) 
\end{align}
We want to know how the ``magnitude'' of the group transformation parameters affect the deviation of $x$. 
Choose a small group element in the vicinity of identity such that $\pi(g) = I + \epsilon^i L_i$.
Expanding to first order in $\epsilon$ we have 
\begin{align}
    \rho(g,x) &= D(E(x)+ \epsilon^iL_i E(x))\cr 
    & \approx D(E(x)) +  \epsilon^iL_i E(x) D'(E(x)) + O(\epsilon^2) \cr
    & = x+ \delta x + \epsilon^iL_i E(x) D'(E(x))
    \label{eq:lat-lin-act}
\end{align}
\nd{One argument for improved long-term forecasting may be related to conservation laws. 
Basically, because of each symmetry, the dynamics has to be orthogonal to some directions ( something like $\nabla Q\cdot dx/dt = 0$?). 
This restricts the subspace on which the dynamics is flowing. 
Can we argue that this leads to slower error growth? }
What if we assume the dynamics is expressed by some nonlinear function $x(t) = F(x_0,t)$? 
The error for $\Delta t$ forecast would come from a Taylor expansion 
\begin{align}
    x(t+\Delta t)= \sum_{k=0}^\infty {\Delta t^k\over k!} {d^k \over d t^k} x(t) 
    \label{eq:F-taylor}
\end{align}
If time translation becomes linear in the AE latent space, what changes? 
For a linear action in the latent space we have \eqref{eq:lat-lin-act}. 
More explicitly
\begin{align}
    \rho(g,x) %&= D(E(x)+ \epsilon^iL_i E(x))\cr 
    & \approx \sum_{k=0}^\infty  \frac{(\epsilon\cdot L E(x))^k}{ k!}  {d^k\over d z^k}D(z)\bigg|_{z=E(x)} 
    \label{eq:lat-lin-taylor}
\end{align}
Calling the time translation Lie algebra basis $H$, we have  
\begin{align}
    x(t+\Delta t) 
    & \approx \sum_{k=0}^\infty  {(\Delta t H z)^k\over k!}  {d^k\over d z^k}D(z)\bigg|_{z=E(x(t))} 
    \label{eq:lat-H-taylor}
\end{align}
So what is the difference between this way of translating time vs. directly Taylor expanding $F$? 
If we compare order $\Delta t^k$ terms in \eqref{eq:F-taylor} with \eqref{eq:lat-H-taylor} we have $x^{(k)}(t) $ in the former and $(Hz)^k D^{(k)}(z)|_{z=E(x)}$ in the latter. 
How can we compare the amount of error accrued in each, if the parameter predictions are slightly off? 
\nd{Maybe it has something to do with the error in prediction being split between $E$ and $D$? 
In the original $x(t)$, the error in a $\delta t$ forecast would come from errors in derivatives $x^{(k)}$. 
With AE, the error burden is on derivatives $D^{(k)}$, linear operator $H$ and $E$, but not derivatives of $E$. 
Could that have a positive effect? 
Like, if we split a function into two parts, could it reduce the rate of error? 
Does the fact that $D \approx E^{-1}$ play a role. 
Naively, the splitting could help, like $x = t^2$ being split into $D= t$ and $E=t$ and only derivatives of one of them mattering? 
Of course this is not the right example, because $D$ and $E$ are not the inverse of each other. 
}

\nd{what should we compare this change with? 
This is what we get when the group action uses an AE. 

}



\section{LieGAN conservation law}
% \newcommand{\Lag}{\mathscr{L}}

% \begin{align}
%     {dQ_i\over dt} = \bk{{d\theta \over dt} , {\ro Q\over \ro \theta}  } = - \bk{\eps \del_\theta \L , \del_\theta  Q  }
% \end{align}

Given data $x\in \mathcal{X}$, LieGAN discovers Lie algebra elements $L_i$ such that for $ g = \exp[t^iL_i]$, $gx $ is also in $\mathcal{X}$, or similar to elements in $\mathcal{X}$. 

Suppose we are learning dynamics with a model equivariant under the symmetries discovered by LieGAN. 
Let $x(t)$ be the positions of the particles at time $t$. 

\newcommand{\Lag}{\mathscr{L}}
First, Noether's theorem states that if the dynamics is derived from a Lagrangian $\Lag$, for each $L_i$, the Noether charge $Q_i$ is conserved during the dynamics, where
\begin{align}
    Q_i&\equiv \bk{L_i x, {\ro \Lag\over \ro v } }, \qquad  
    {dQ_i\over dt} = 0  
    \label{eq:Noether-Lagrange}
\end{align}
where $v = \dot{x} = dx/dt$ are the velocities. 
However, using \eqref{eq:Noether-Lagrange} requires knowing the Lagrangian, which we often do not have. 
From the definition of momentum $p$ in  Hamiltonian dynamics, we have
\begin{align}
    p & \equiv {\ro \Lag\over \ro v }, \qquad
    \Rightarrow\qquad 
    Q_i = \bk{L_i x , p} 
    \label{eq:Noether-Hamilton}
\end{align}
Hence, if we have access to momenta, we can directly compute Noether's charges $Q_i$ from \eqref{eq:Noether-Hamilton}. 

\subsection{More general case without Lagrangian}
If we have neither the momenta $p$ nor the Lagrangian $\Lag$, we need to make assumptions about $\Lag$ in order to find a Noether charge $Q_i$. 
The simplest assumption for the form of the Lagrangian is to assume it consists of a kinetic energy term $K(v)$ and a potential energy $V(x)$, which holds for many physical systems
\begin{align}
    \Lag(x,v) &= K(v)- V(x) = {m\over 2} \eta_{\mu\nu} v^\mu v^\nu - V(x)
    \label{eq:Lag-K-V}
\end{align}
where $\eta_{\mu\nu}$ are componenets of metric of space (or space-time), and $m$ is the mass of the particles. 
Using \eqref{eq:Lag-K-V}, the momentum $p$ is given by
\begin{align}
    p & = {\ro \Lag\over \ro v } = m\eta v, \qquad
    \Rightarrow\qquad 
    Q_i = \bk{L_i x , m\eta {dx\over dt} }.  
    \label{eq:Noether-Hamilton}
\end{align}
We may approximate the velocities $v=dx/dt$ from $x(t)$ of consecutive time steps. 
If all particles have the same mass, we can neglect $m$, as a constant factor in $Q_i$ doesn't matter. 
However, if the particles have different masses, we either need to know $m$, or somehow learn the masses. 

We also have a procedure for finding the metric $\eta$ using $L_i$ by requiring $\eta$ is invariant under $G$, which yields $L_i^T \eta + \eta L_i = 0 $. 
Note that the ansatz in \eqref{eq:Lag-K-V} doesn't work for electromagnetism, or systems with friction, or fluids with viscosity. 


\newpage



